ApplicaAI at SemEval-2020 Task 11: On RoBERTa-CRF, Span CLS and Whether Self-Training Helps Them

This paper presents the winning system for the propaganda Technique Classification (TC) task and the second-placed system for the propaganda Span Identification (SI) task. The purpose of TC task was to identify an applied propaganda technique given propaganda text fragment. The goal of SI task was to find specific text fragments which contain at least one propaganda technique. Both of the developed solutions used semi-supervised learning technique of self-training. Interestingly, although CRF is barely used with transformer-based language models, the SI task was approached with RoBERTa-CRF architecture. An ensemble of RoBERTa-based models was proposed for the TC task, with one of them making use of Span CLS layers we introduce in the present paper. In addition to describing the submitted systems, an impact of architectural decisions and training schemes is investigated along with remarks regarding training models of the same or better quality with lower computational budget. Finally, the results of error analysis are presented.

==> inputs/hp-finetune-both.tex <==
\begin{subtable}{\linewidth}
   \centering
   \input{inputs/hp-finetune}
   \vspace{3mm}
\end{subtable}
\begin{subtable}{\linewidth}
   \centering
   \input{inputs/hp-finetune-self}
\end{subtable}%
\caption{
    Optimizers and hyperparameters used for both finetuning RoBERTa and training additional parameters.
}

==> inputs/schreirer-ray-hare.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{cccc}
    \toprule
    \bf model & \bf H & \bf p-value & \bf significance \\
    \midrule
    (1) & $18.69$ & $<0.001$ & 1\\
    (2) & $23.58$ & $<0.001$ & 1\\
    (3) & $15.23$ & $<0.001$ & 1\\
    (4) & $35.01$ & $<0.001$ & 1\\
    (5) & $27.50$ & $<0.001$ & 1\\
    (6) & $3.33$ & $0.068$ & 0\\
    (7) & $62.06$ & $<0.001$ & 1\\
    (8) & $29.17$ & $<0.001$ & 1\\
    \bottomrule
\end{tabular}
\caption{Schreirer-Ray-Hare test. p-value lower than 0.05 leads to the rejection of null hypotheses stating that ensemble components have no influence on the score.}
\label{tab:schreirer-tc}

==> inputs/span-cls.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/span_cls.pdf}
    \caption{Classification of text span with Span CLS. In this approach small transformer is stacked over the selected tokens only. It has no own embeddings apart from one for \texttt{[BOS]} token, but uses representations provided by the host model instead.}
    \label{fig:span_cls}
\end{figure}

==> inputs/spearman-tc.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{cc}
    \toprule
    \bf Model & \bf $\bm{\rho}$  \\
    \midrule
    (1) & $0.28$ \\
    (2) & $0.30$ \\
    (3) & $0.20$ \\
    (4) & $0.41$ \\
    (5) & $0.32$ \\
    (6) & $0.05$ \\
    (7) & $0.50$ \\
    (8) & $0.36$ \\
    \bottomrule
\end{tabular}
\caption{Spearman correlation between presence of ensemble components (models from Table~\ref{tab:scores-tc}) and score achieved by the ensemble.}
\label{tab:spearman-tc}

==> inputs/special-tokens.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/special_tokens.pdf}
    \caption{Classification of text span by means of introduced special \texttt{[BOP]} and \texttt{[EOP]} tokens. Span is further classified as in usual transformer-based sentence classification task.}
    \label{fig:special_tokens}
\end{figure}


==> keywords.tex <==
some keyword, another keyword

